HSFM-$\Sigma$nn: Combining a Feedforward Motion Prediction Network and Covariance Prediction

In this paper, we propose a new method for motion prediction: HSFM-$\Sigma$nn. Our proposed method combines two different approaches: a feedforward network whose layers are model-based transition functions using the HSFM and a Neural Network (NN), on each of these layers, for covariance prediction. We will compare our method with classical methods for covariance estimation showing their limitations. We will also compare with a learning-based approach, social-LSTM, showing that our method is more precise and efficient.

==> inputs/method.tex <==
\section {Approach}
\TODO{I started again on this, see method2}
In this part, we will describe which algorithms and methods we use for choosing meaningful robot behaviour in a highly dynamic environment.

\subsection{Riskaware Backprop-MPDM}

In our work we use MPDM with backward optimization over probabilistic cost, in order to choose best policy, wrt. to cost, over a predefined set of policies. In a risk aware MPDM, the robot`s policies are evaluated based on the most influential outcome that may occur, with such an approach we can evaluate the most dangerous outcome for each policy, and choose the safest one among all possible policies. In order to evaluate such outcomes we use probabilistic cost surface  %$max{...}$,  where  …. P = .. C =  .. X = …
\begin{equation}
    max_{x_{0}}(P(x_{0})C(X(\pi,x_{0})))
\end{equation}
\begin{equation}
C(X(\pi,x_{0})) = Blame(X) + Progress(X)
\end{equation}
Where $x_{0}$ is initial sampled configuration of environment, including robot pose and all observed pedestrian poses, $\pi=(v_{des},g_{sub})$ is an agent policy, describing intent to move toward subgoal $g_{sub}$ at desired speed $v_{des}$,  - outcome cost of simulation, where $Blame(X(\pi,x_{0}))$ penalizes the inconvenience the robot causes to other agents,

\begin{figure}[htbp]
\centerline{\includegraphics[scale=0.3]{images/icra text (1).png}}
\caption{Representation of transition function for forward simulation}
\label{fig}
\end{figure}

and $Progress(X(\pi,x_{0}))$ is rewards the robot’s progress towards its goal.

\subsection{Trajectory prediction}

In order to calculate cost and choose optimal policy, MPDM algorithms need accurate trajectories predictions. Recently there appeared a number of new approaches for this task. In order to maximise possible number of evaluated policies, we are interested in both accuracy and processing time of prediction algorithms. In our work we use  Headed-Social Force Model (HSFM) and social-LSTM models. SFM for a long time was a classical approach for  trajectories prediction, with low computational costs. However, modern deep approaches are showing more accurate predictions, and some of them has fast inference time. 

Block diagram of the transition function depicted in fig. 1. During forward simulation current state of robot $x^{r}_{t-1}$ and current states of all pedestrians $x^{1..N}_{t-1}$ are passed as input to the transition function. This data is processed by HSFM or LSTM modules, depending on the chosen algorithm. Then output of processing cells are transformed to predicted coordinates by human locomotion model in case of HSFM or by pre-trained Linear model in case of LSTM algorithm. 
Unicycle kinematic transformation can be calculated as:
\begin{equation}
\begin{bmatrix}
v_{ref} \\
\omega_{ref}\\
\end{bmatrix}
_{t+1}=
\begin{bmatrix}

cos(\theta)& sin(\theta) &   \\
- sin(\theta) & cos(\theta \\
\end{bmatrix} 
\begin{bmatrix}
1 & 0 \\
0 & \frac{1}{l} \\
\end{bmatrix} 
f^{r}_{net}
\end{equation}
Where $v_{ref}$ - linear velocity of robot,  $w_{ref}$ - angular velocity, $\theta$ - orientation, $f^{r}_{net}$ - resulting vector of forces calculated by HSFM module.


\subsection{Cost optimization}

In Backprop-MPDM[] has been shown that it is possible and effective to conceptualize the forward simulation, as a number of stacked transition functions (fig 1) that outputs predicted state of all pedestrians and robot at timestamp $t+1$ together with trajectory cost at this timestamp $C(X(x_{0}))$.
\newline
Our used transition function  $T (x_{t})$ (Fig. 1) allows us to compute accurate gradients of the transition Function. Gradients calculation are implemented via back-propagation, where  $\frac{\delta L}{\delta x}$ is computed during the forward propagation. 
\newline
\begin{equation}
    \bigtriangledown _{x_{0}} L(X) = \bigtriangledown _{x_{0}} P(x)C(X(x_{0} , \pi_{r} ))
\end{equation}{}

The gradient of the cost function with respect to the agent configurations(eqn. 4) is used during gradient-ascent to simultaneously perturb the configurations of all pedestrians towards increasingly likely and high-cost outcomes until convergence.




% \begin{figure}[h]

% \begin{subfigure}{0.5\textwidth}
% \includegraphics[width=0.9\linewidth, height=5cm]{images/mpdh_hsfm.png} 
% \caption{Caption1}
% \label{fig:subim1}
% \end{subfigure}
% \begin{subfigure}{0.5\textwidth}
% \includegraphics[width=0.9\linewidth, height=5.5cm]{images/mpdm_full2.png}
% \caption{Visualization of simulation. Here grey ellipsoids represents simulated pedestrians, green ellipsoid represents controlled robot. Purple translucent ellipsoids - trajetories of each agent in scene predicted by HSFM, squres - trajetories of each agent in scene predicted by social-LSTM. "go-solo" on top of robot pose represents chosen policy, according to performed si,ulation process}
% \label{fig:subim2}
% \end{subfigure}
% \caption{Caption for this figure with two images}
% \label{fig:image2}
% \end{figure}



==> inputs/old.tex <==
\subsection{Abbreviations and Acronyms}\label{AA}
Define abbreviations and acronyms the first time they are used in the text, 
even after they have been defined in the abstract. Abbreviations such as 
IEEE, SI, MKS, CGS, ac, dc, and rms do not have to be defined. Do not use 
abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}
\begin{itemize}
\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
\item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
\end{itemize}

\subsection{Equations}
Number equations consecutively. To make your 
equations more compact, you may use the solidus (~/~), the exp function, or 
appropriate exponents. Italicize Roman symbols for quantities and variables, 
but not Greek symbols. Use a long dash rather than a hyphen for a minus 
sign. Punctuate equations with commas or periods when they are part of a 
sentence, as in:
\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

Be sure that the 
symbols in your equation have been defined before or immediately following 
the equation. Use ``\eqref{eq}'', not ``Eq.~\eqref{eq}'' or ``equation \eqref{eq}'', except at 
the beginning of a sentence: ``Equation \eqref{eq} is . . .''

\subsection{\LaTeX-Specific Advice}

Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.

\section*{Acknowledgment}

The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.

\section*{References}

Please number citations consecutively within brackets \cite{b1}. The 
sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

Number footnotes separately in superscripts. Place the actual footnote at 
the bottom of the column in which it was cited. Do not put footnotes in the 
abstract or reference list. Use letters for table footnotes.

Unless there are six authors or more give all authors' names; do not use 
``et al.''. Papers that have not been published, even if they have been 
submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
Capitalize only the first word in a paper title, except for proper nouns and 
element symbols.

For papers published in translation journals, please give the English 
citation first, followed by the original foreign-language citation \cite{b6}.

\begin{thebibliography}{00}
\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
\end{thebibliography}
\vspace{12pt}
\color{red}
IEEE conference templates contain guidance text for composing and formatting conference papers. Please ensure that all template text is removed from your conference paper prior to submission to the conference. Failure to remove the template text from your paper may result in your paper not being published.


==> inputs/related.tex <==
\section{Related Work}

In our work we are interesting in covariance estimation for pedestrians trajectories prediction, in this section we will briefly discuss later advances in these research areas.


% second taxonomy single point vs distribution

\subsection{Trajectory prediction}

Recently there has been a number of different deep learning approaches to predict pedestrians trajectories.  Human trajectory prediction using deep models Social-LSTM \cite{Alahi} - proposes LSTM model with developed pooling method which jointly predicts the trajectories of all the people in a scene, in order to model the human-human interactions. Predicted parameters are assumed to be parameters of Gaussian distribution: mean $\mu^{i}_{t+1}  = (\mu +{x}, \mu _{y})^{i}_{t+1}$, standard deviation $\sigma^{i}_{t+1}  = [\sigma _{x}, \sigma _{y}]^{i}_{t+1}$ and correlation coefficient $ p ^{i}_{t+1}$. These parameters are predicted by a linear layer.

\texttt{Zhang} at \texttt{State-Refinement LSTM} \cite{Zhang} by comparison with the Vanilla LSTM \cite{Alahi} applied  states refinement module, which adaptively focuses on the most useful neighboring information and guide the message passing, with a social-aware information selection mechanism.

\texttt{Agrim Gupta} at \texttt{Social-GAN} \cite{Gupta} show how GAN based architectures might be applied pedestrian trajectories prediction networks. In these work they predict socially plausible futures by training adversarially against





% Metha and Ferrer at Backprop-MPDM: Faster risk-aware policy evaluation through efficient gradient optimization[] showed that accurate gradients can be computed – even through a complex forward simulation – using approaches similar to those in deep networks. We show that our proposed approach finds influential outcomes more reliably,
% and is faster than earlier  methods, allowing us to evaluate more policies while simultaneously eliminating the need to design an easily-differentiable heuristic function.




% \TODO{this section should be out, no navigation, only as an application for prediction}
% \subsection{Navigation in dynamic and uncertain environments}
% MPDM is a high-level decision making process that factors autonomous driving into a set of policies that encode closed loop behaviors and uses online simulation to evaluate the consequences of available policies. 

% Cunningham and others  at MPDM: Multipolicy Decision-Making in Dynamic,
% Uncertain Environments for Autonomous Driving[] introduced are general pipeline for the problem of decision-making in dynamic, uncertain environments with tight coupling between the actions of multiple agents.


% Autorhs of Fast discovery of influential outcomes for risk-aware MPDM[]  in their work introduced a risk-aware approach for MPDM, and developed a cost function based on two components: Blame - captures the potential inconvenience that the robot might cause in the environment and Progress - indicates progress made towards the goal. For finding pseudo-optimal solution authors used the Stochastic Gradient Ascent algorithm in order to minimize cost function in forward simulations. 



% \begin{figure}[htbp]
% \centerline{\includegraphics[scale=0.3]{images/mpdm_full2.png}}
% \caption{Visualization of simulation. Here grey ellipsoids represents simulated pedestrians, green ellipsoid represents controlled robot. Purple translucent ellipsoids - trajectories of each agent in scene predicted by HSFM, squares - trajectories of each agent in scene predicted by social-LSTM. "go-solo" on top of robot pose represents chosen policy, according to performed simulation process}
% \label{fig}
% \end{figure}
